HODA: Hardness-Oriented Detection of Model Extraction Attacks

Model Extraction attacks exploit the target model's prediction API to create a surrogate model in order to steal or reconnoiter the functionality of the target model in the black-box setting. Several recent studies have shown that a data-limited adversary who has no or limited access to the samples from the target model's training data distribution can use synthesis or semantically similar samples to conduct model extraction attacks. In this paper, we define the hardness degree of a sample using the concept of learning difficulty. The hardness degree of a sample depends on the epoch number that the predicted label of that sample converges. We investigate the hardness degree of samples and demonstrate that the hardness degree histogram of a data-limited adversary's sample sequences is distinguishable from the hardness degree histogram of benign users' samples sequences. We propose Hardness-Oriented Detection Approach (HODA) to detect the sample sequences of model extraction attacks. The results demonstrate that HODA can detect the sample sequences of model extraction attacks with a high success rate by only monitoring 100 samples of them, and it outperforms all previous model extraction detection methods.

==> content/detailaeattack.tex <==
\label{sec:detailatt}
We employ Adversarial Robustness Toolbox (ART)\footnote{https://github.com/Trusted-AI/adversarial-robustness-toolbox} and AutoAttack\footnote{https://github.com/fra31/auto-attack} repositories to generate adversarial examples. Except for attacks' hyperparameters being mentioned in the following, we use the default values for the rest of the hyperparameters. All attacks generate untargeted adversarial examples in the white-box setting. The success rates of attacks are presented in Table \ref{tab:advexattsucrate}.

\textbf{Fast Gradient Sign Method (FGSM)} \cite{DBLP:journals/corr/GoodfellowSS14}: FGSM is a one-step attack that uses $L_{\infty}$-norm to control the magnitude of perturbations being added to normal samples. This attack calculates the gradient of the loss function with respect to the input and takes one step with size $\epsilon$ in the gradient's direction.
\begin{equation}
x' = x + \epsilon.sign(\nabla_x\mathcal{L}(\theta,x,y))
\end{equation}
 We use $\epsilon=0.1$ to generate adversarial examples.
 
 \textbf{Carlini and Wagner (C\&W)} \cite{DBLP:conf/sp/Carlini017}: Carlini and Wagner propose an iterative attack to break defensive distillation \cite{7546524}. They propose three variants of their attack based on $L_0$, $L_2$, and $L_\infty$-norms. In the $L_2$-norm attack, adversarial examples are generated by minimizing the following equation:
 \begin{equation}
 \begin{split}
 &\mathcal{D}(x, x+\eta) + c.g(x+\eta) \\
 &s.t. \quad x + \eta \in Domain(x)
 \end{split}
 \end{equation}
 where $\mathcal{D}(x)$ in $L_2$-norm and $g(x)$ is the objective function. The authors consider several objective functions and pick one of them based on the experiments.
 We use $L_2$-norm variant to generate adversarial examples in five iterations and use five binary search steps to select $c$.
 
 \textbf{Projected Gradient Decent (PGD)} \cite{DBLP:conf/iclr/MadryMSTV18}: PGD is an iterative method that improves FGSM to generate more powerful adversarial examples. In each iteration, PGD takes one step with size $\alpha$ in the direction of loss function gradient with respect to the input. It uses projection $\Pi_\epsilon$ to restrict the $L_{\infty}$-norm of perturbation to $\epsilon$.
 \begin{equation}
 x^{t+1} = \Pi_\epsilon(x^t + \alpha.sign(\nabla_x\mathcal{L}(\theta,x,y)) 
 \end{equation}
 We use 50 iterations to generate each adversarial example with $\alpha=\frac{3}{255}$ and $\epsilon=\frac{8}{255}$.
 
 \textbf{AutoAttack (AA)} \cite{DBLP:conf/icml/Croce020a}: AA using some techniques, such as step size selection, improves the performance of PGD attack. AA is a parameter-free attack. We use $L_{\infty}$-norm to restrict the size of perturbation and $\epsilon=\frac{8}{255}$ to generate adversarial examples.

\begin{table}[]
	\caption{Adversarial example attacks success rate.}
		\vspace{-0.6\baselineskip}
	\label{tab:advexattsucrate}
\begin{tabular}{ccccc}
	& \multicolumn{4}{c}{Attack Success Rate (\%)} \\ \cline{2-5} 
	& FGSM       & C\&W      & PGD      & AA       \\ \hline
	CIFAR10  & 84.3       &    90.9      & 100      & 100      \\
	CIFAR100 & 97.0       & 97.8      & 100      & 100     
\end{tabular}
\end{table}



==> content/detectaehighprec.tex <==
\label{sec:detectadvexampleseqappendix}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!t]
	\caption{The detection rate and False Positive Rate (PFR) of HODA against four various adversarial example attacks. HODA uses 100 subclassifiers to calculate the hardness degree of samples.
		The FPR indicates the percentage of benign users' sample sequences that are detected as sample sequences of attacks.  
		AE percentage indicates what percentage of adversaries' sample sequences are adversarial examples.}
			\vspace{-1.0\baselineskip}
	\label{tab:aedetectratehundered}
	\renewcommand{\arraystretch}{1.0}
	\resizebox{\linewidth}{!}{
		\begin{tabular}{ccccccc}
			&                                                                                 &     & \multicolumn{4}{c}{Detection Rate of Attacks(\%)} \\ \cline{4-7} 
			&                                                          & {\begin{tabular}[c]{@{}c@{}}AE \\ Percentage(\%)\end{tabular}}  & FGSM      & C\&W     & PGD       & AA     \\ \hline
			\multirow{8}{*}{\rotatebox{90}{CIFAR10}}  & \multirow{4}{*}{\begin{tabular}[l]{@{}l@{}}$num_{s}$: 100\\ $\delta$: 0.164\\ FPR: 0.04\%\end{tabular}} & 10  & 0.02      &      0.08         & 0.2      & 0.2       \\
			&                                                                                 & 25  & 1.8      &        11.8       & 10.4      & 21.5     \\
			&                                                                                 & 50  & 96.6      &       99.9        & 97.1     & 99.1     \\
			&                                                                                 & 100 & 100       &       100        & 100       & 100       \\ \cline{2-7} 
			& \multirow{4}{*}{\begin{tabular}[l]{@{}l@{}}$num_s$: 500\\ $\delta$: 0.022\\ FPR: 0.07\%\end{tabular}} & 10  & 0.12      &         0.89      & 15.35      & 31.1      \\
			&                                                                                 & 25  & 83.3      &        99.9       & 99.9      & 99.5     \\
			&                                                                                 & 50  & 100       &       100        & 100       & 100       \\
			&                                                                                 & 100 & 100       &      100         & 100       & 100       \\ \hline
			\multirow{8}{*}{\rotatebox{90}{CIFAR100}} & \multirow{4}{*}{\begin{tabular}[l]{@{}l@{}}$num_s$: 100\\ $\delta$: 0.660\\ FPR: 0.01\%\end{tabular}}  & 10  & 0.03      &      0.16         & 0.02      & 0.03      \\
			&                                                                                 & 25  & 3.2      &          10.6     & 0.3      & 0.3      \\
			&                                                                                 & 50  & 74.6     &       98.8        & 11.2     & 13.7     \\
			&                                                                                 & 100 & 99.8     &      100         & 97.4    & 99.1     \\ \cline{2-7} 
			& \multirow{4}{*}{\begin{tabular}[l]{@{}l@{}}$num_s$: 500\\ $\delta$: 0.144\\ FPR: 0.03\%\end{tabular}} & 10  & 2.3      &       21.6        & 3.2      & 1.9       \\
			&                                                                                 & 25  & 94.6     &         100      & 97.3     & 85.7     \\
			&                                                                                 & 50  & 100       &        100       & 100       & 100       \\
			&                                                                                 & 100 & 100       &       100        & 100       & 100      
		\end{tabular}
	}
\end{table}

Table \ref{tab:aedetectratehundered} shows the performance of HODA against four adversarial examples attacks when HODA uses 100 subclassifiers to calculate the hardness degree of samples. 
We observed that when we use hardness degree histograms that have 10 bins rather than 100 bins, the performance of HODA is increased. Hence, although the hardness degree of samples is in the range [0,99], we divide the hardness degree of samples by 10 to the number of bins in hardness degree histograms decreases to 10.



==> content/dnns.tex <==
\label{sec:dl}
A Deep Neural Network (DNN)-based classifier is a hierarchical function $f:\mathcal{X} \rightarrow \mathcal{Y}$ that maps the input space $\mathcal{X}$ to the output space $\mathcal{Y}$. DNNs have multiple layers that each layer includes an affine transformation followed up by a non-linear function called activation function. 
Each DNN has a parameter set $\theta$ being tuned during the training process to minimize the loss function $\mathcal{L}$ on the training set $\mathbb{X}$. The training set $\mathbb{X}=\{(x_i,y_i)\}^{N}_{i=1}$ consists of $N$ pairs that each pair includes a sample $x_i \in \mathbb{R}^d$ and the corresponding label $y_i \in [K]$, where $d$ is the input's dimension, and $K$ is the number of classes. The output of classifier $\hat{y}_i = f(x_i)$ is a probability vector over K classes. The $j^{th}$ element of $\hat{y}_i$ indicates the classifier's confidence that $x_i$ belongs to the $j^{th}$ class. Hence, the label of data $x_i$ is $argmax(f(x_i))$.
The loss function $\mathcal{L}$ is used to calculate the distance between label $y_i$ and the output of classifier $\hat{y}_i=f(x_i)$ for sample $x_i$. The minimization of loss function $\mathcal{L}$ is usually done using some common versions of the Stochastic Gradient Descent (SGD). SGD is an iterative algorithm that initializes the classifier's parameters randomly and then takes a step in the inverse direction of the gradient of loss function with respect to the classifier's parameters in each iteration.
\begin{equation}
\theta_{t+1} = \theta_{t} - \eta_t \frac{\partial \mathcal{L}}{\partial \theta}
\end{equation}
where $\eta_t$ is learning rate that regulates the size of steps and is often scheduled to be decreased during the training process. 
Most often, SGD is run for multiple epochs.  All samples in the training set are shuffled and then are partitioned into several mini-batches in each epoch. SGD uses each mini-batch to calculate loss function and updates classifier's parameters for one step. There are some heuristic methods that determine the number of epochs. However, the number of training epochs is often considered as a hyperparameter and it is determined before the training phase. After the training process is done, the classifier is evaluated on unseen samples in the training phase, which is called test set, to determine the true performance of classifier in practice. For simplicity, we use classifier instead of DNN-based classifier in the rest of the paper.




==> content/figure/corrmodels.tex <==

\begin{figure*}
	\centering
	\begin{subfigure}{\linewidth}
		\centering
		\resizebox{\linewidth}{!}{
	\begin{tikzpicture}
	\begin{groupplot}[group style={group size= 4 by 1,horizontal sep = 1cm,group name=my plots,},height=4.5cm,width=4.5cm,tick label style = {font = {\fontsize{6 pt}{12 pt}\selectfont}},]
	\nextgroupplot[
	enlargelimits=false,
	title= \scriptsize{(A) ResNet18 - (B) ResNet18},
	ylabel= \scriptsize{Hardness Rank (A)},
	ytick = {0,1000,2000,3000,4000,5000},
	yticklabels={0,1K,2K,3K,4K,5k},
	xtick = {0,1000,2000,3000,4000,5000},
	xticklabels={0,1K,2K,3K,4K,5k},
	]
	\addplot[
	scatter/classes={
		a={mark=*,blue},
		b={mark=*,blue},
		c={mark=*,blue},
		d={mark=*,blue}
	},
	scatter, only marks,
	scatter src=explicit symbolic,
	mark size = 0.01pt]
	table[x=x,y=y,meta=label]
	{resrescifar10.dat};
	
	\nextgroupplot[
enlargelimits=false,
title= \scriptsize{(A) ResNet18 - (B) DenseNet121},
	ytick = {0,1000,2000,3000,4000,5000},
yticklabels={0,1K,2K,3K,4K,5k},
xtick = {0,1000,2000,3000,4000,5000},
xticklabels={0,1K,2K,3K,4K,5k},
]
\addplot[
scatter/classes={
	a={mark=*,blue},
	b={mark=*,blue},
	c={mark=*,blue},
	d={mark=*,blue}
},
scatter, only marks,
scatter src=explicit symbolic,
mark size = 0.01pt]
table[x=x,y=y,meta=label]
{resdenscifar10.dat};

	\nextgroupplot[
enlargelimits=false,
title= \scriptsize{(A) ResNet18 - (B) MobileNet},
	ytick = {0,1000,2000,3000,4000,5000},
yticklabels={0,1K,2K,3K,4K,5k},
xtick = {0,1000,2000,3000,4000,5000},
xticklabels={0,1K,2K,3K,4K,5k},
]
\addplot[
scatter/classes={
	a={mark=*,blue},
	b={mark=*,blue},
	c={mark=*,blue},
	d={mark=*,blue}
},
scatter, only marks,
scatter src=explicit symbolic,
mark size = 0.01pt]
table[x=x,y=y,meta=label]
{resmobcifar10.dat};

	\nextgroupplot[
enlargelimits=false,
title= \scriptsize{ (A) DenseNet121 - (B) MobileNet},
	ytick = {0,1000,2000,3000,4000,5000},
yticklabels={0,1K,2K,3K,4K,5k},
xtick = {0,1000,2000,3000,4000,5000},
xticklabels={0,1K,2K,3K,4K,5k},
]
\addplot[
scatter/classes={
	a={mark=*,blue},
	b={mark=*,blue},
	c={mark=*,blue},
	d={mark=*,blue}
},
scatter, only marks,
scatter src=explicit symbolic,
mark size = 0.01pt]
table[x=x,y=y,meta=label]
{denmobcifar10.dat};
	\end{groupplot}
\end{tikzpicture}
}
\vspace{-0.5cm}
\caption{ Cifar10}
	\end{subfigure}

\begin{subfigure}{\linewidth}
\centering
\hspace{0cm}
\resizebox{\linewidth}{!}{
\begin{tikzpicture}
	\begin{groupplot}[group style={group size= 4 by 1,horizontal sep = 1cm,group name=my plots,},height=4.5cm,width=4.45cm,tick label style = {font = {\fontsize{6 pt}{12 pt}\selectfont}},]

	\nextgroupplot[
enlargelimits=false,ylabel= \scriptsize{Hardness Rank (A)},xlabel= \scriptsize{Hardness Rank (B)},
	ytick = {0,1000,2000,3000,4000,5000},
yticklabels={0,1K,2K,3K,4K,5k},
xtick = {0,1000,2000,3000,4000,5000},
xticklabels={0,1K,2K,3K,4K,5k},
]
\addplot[
scatter/classes={
	a={mark=*,blue},
	b={mark=*,blue},
	c={mark=*,blue},
	d={mark=*,blue}
},
scatter, only marks,
scatter src=explicit symbolic,
mark size = 0.01pt]
table[x=x,y=y,meta=label]
{resrescifar100.dat};

	\nextgroupplot[
enlargelimits=false,xlabel= \scriptsize{Hardness Rank (B)},scaled y ticks = false,
	ytick = {0,1000,2000,3000,4000,5000},
yticklabels={0,1K,2K,3K,4K,5k},
xtick = {0,1000,2000,3000,4000,5000},
xticklabels={0,1K,2K,3K,4K,5k},
]
\addplot[
scatter/classes={
	a={mark=*,blue},
	b={mark=*,blue},
	c={mark=*,blue},
	d={mark=*,blue}
},
scatter, only marks,
scatter src=explicit symbolic,
mark size = 0.01pt]
table[x=x,y=y,meta=label]
{resdencifar100.dat};


	\nextgroupplot[
enlargelimits=false,xlabel= \scriptsize{Hardness Rank (B)},
	ytick = {0,1000,2000,3000,4000,5000},
yticklabels={0,1K,2K,3K,4K,5k},
xtick = {0,1000,2000,3000,4000,5000},
xticklabels={0,1K,2K,3K,4K,5k},
]
\addplot[
scatter/classes={
	a={mark=*,blue},
	b={mark=*,blue},
	c={mark=*,blue},
	d={mark=*,blue}
},
scatter, only marks,
scatter src=explicit symbolic,
mark size = 0.01pt]
table[x=x,y=y,meta=label]
{resmobcifar100.dat};

	\nextgroupplot[
enlargelimits=false,xlabel= \scriptsize{Hardness Rank (B)},
	ytick = {0,1000,2000,3000,4000,5000},
yticklabels={0,1K,2K,3K,4K,5k},
xtick = {0,1000,2000,3000,4000,5000},
xticklabels={0,1K,2K,3K,4K,5k},
]
\addplot[
scatter/classes={
	a={mark=*,blue},
	b={mark=*,blue},
	c={mark=*,blue},
	d={mark=*,blue}
},
scatter, only marks,
scatter src=explicit symbolic,
mark size = 0.01pt]
table[x=x,y=y,meta=label]
{denmobcifar100.dat};
	\end{groupplot}
	\end{tikzpicture}
}
	\vspace{-0.5cm}
	\caption{ Cifar100}
\end{subfigure}
\vspace{-0.5\baselineskip}
\caption{Hardness rank of 5000 test samples of CIFAR10 and CIFAR100 datasets for various pairs of classifiers. }
\label{fig:modelscorr}
\end{figure*}






==> content/seclabelhardanalysis.tex <==
\label{sec:labelonlyhardnessanalysis}

Figure \ref{fig:hardnesanalysislabelonly} shows the accuracy and the fidelity of attacks over 10 hardness groups when the output of target classifier is only label.

\input{content/new_labelhardanalysis.tex}





==> content/tm.tex <==
\label{sec:threatmodel}

